Heuristics for Symmetric Rectilinear Matrix Partitioning

Partitioning sparse matrices and graphs is a common and important problem in many scientific and graph analytics applications. In this work, we are concerned with a spatial partitioning called rectilinear partitioning (also known as generalized block distribution) of sparse matrices, which is needed for tiled (or {\em blocked}) execution of sparse matrix and graph analytics kernels. More specifically, in this work, we address the problem of symmetric rectilinear partitioning of square matrices. By symmetric, we mean having the same partition on rows and columns of the matrix, yielding a special tiling where the diagonal tiles (blocks) will be squares. We propose five heuristics to solve two different variants of this problem, and present a thorough experimental evaluation showing the effectiveness of the proposed algorithms.

==> Makefile <==
PAPER = paper
VERBOSE = 0

# directories
FIGURE_DIR = ./figures
OUTPUT_DIR = ./output
STYLE_DIR = ./style
TEXT_DIR = ./
BIB_OUT_FILE = $(OUTPUT_DIR)/bib-issues

# paths
BIB_PATH="$(TEXT_DIR)"
BST_PATH="$(STYLE_DIR)/sty:$(shell kpsewhich --progname=latex --show-path=.bst)"
TEX_PATH="$(TEXT_DIR):$(STYLE_DIR):$(STYLE_DIR)/sty:$(shell kpsewhich -progname=tex -show-path=tex)"

# options
BIBTEX_OPTS = -terse
DVIPS_OPTS = -q -G0 -tletter
LATEX_OPTS  = -output-directory=$(OUTPUT_DIR) -file-line-error -interaction=batchmode
MAKEINDEX_OPTS = -q
PS2PDF_OPTS = -q -sPAPERSIZE=letter -dSAFER -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -dPDFSETTINGS=/prepress \
              -dCompatibilityLevel=1.4 -dMaxSubsetPct=100 -dSubsetFonts=true

#commands
LATEXC = max_print_line=1000 pdflatex
PRINT_LATEX_ERRORS = (cat $(OUTPUT_DIR)/$(PAPER).log | grep '^[^: ]*:[^: ]*:' || exit 0)
PRINT_LATEX_WARNINGS = (cat $(OUTPUT_DIR)/$(PAPER).log | sed -n '1h;1!H;$${;g;s/\n / /g;p;}' | grep -i 'latex warning' || exit 0)
PRINT_BIBTEX_WARNINGS = (cat $(OUTPUT_DIR)/*.blg | grep '^Warning' | sort | uniq > $(BIB_OUT_FILE) || exit 0)

#formats
NORM=
BOLD=
PS2PDF_LABEL   =[ps2pdf   ]
DVIPS_LABEL    =[dvips    ]
LATEX_LABEL    =[pdflatex ]
BIBTEX_LABEL   =[bibtex   ]
NOTE_LABEL     =[note     ]
MAKEINDEX_LABEL=[makeindex]
RM_LABEL       =[rm       ]

SHELL:=/bin/bash

all: $(OUTPUT_DIR)/$(PAPER).pdf

show: $(OUTPUT_DIR)/$(PAPER).pdf
	@open $(OUTPUT_DIR)/$(PAPER).pdf &

$(OUTPUT_DIR)/$(PAPER).pdf: $(TEXT_DIR)/$(PAPER).tex                     \
                           $(shell find $(TEXT_DIR) -regex "[^.]*.tex")  \
                           $(shell find $(TEXT_DIR) -regex  "[^.]*.bib") \
                           $(shell find $(STYLE_DIR) -regex "[^.]*.tex") \
                           $(shell find $(FIGURE_DIR) -name "*.pdf")
	@mkdir -p $(OUTPUT_DIR)

	@echo "$(LATEX_LABEL)Performing initial latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

	@echo "$(BIBTEX_LABEL)Processing bibliography..."
	@BIBINPUTS=$(BIB_PATH) \
	 BSTINPUTS=$(BST_PATH) \
		bibtex $(BIBTEX_OPTS) output/$(PAPER) | grep -v "^Warning"; \
		if [ $${PIPESTATUS[0]} != 0 ]; then \
			rm -f $@ && exit 1; \
		fi
	@-$(PRINT_BIBTEX_WARNINGS)
	@echo "$(NOTE_LABEL)Bibliography warnings written to '$(BIB_OUT_FILE)'."

#	@echo "$(MAKEINDEX_LABEL)Building index..."
#	@makeindex $(MAKEINDEX_OPTS) $(OUTPUT_DIR)/$(PAPER).idx || \
#		(rm -f $@ && exit 1)

	@echo "$(LATEX_LABEL)Performing secondary latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

#	@echo "$(LATEX_LABEL)Performing ternary latex..."
#	@TEXINPUTS=$(TEX_PATH) \
#		latex $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
#			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)

	@echo "$(LATEX_LABEL)Performing final latex..."
	@TEXINPUTS=$(TEX_PATH) \
		$(LATEXC) $(LATEX_OPTS) $(PAPER).tex >/dev/null || \
			(rm -f $@ && $(PRINT_LATEX_ERRORS) && exit 1)
	@-$(PRINT_LATEX_WARNINGS)

clean:
	@echo '$(RM_LABEL)Cleaning project...'
	@rm -fr $(OUTPUT_DIR)
